AdaDINO: Context-Adaptive DINO-Distilled Vision Foundation Models for Efficient Open-Vocabulary Edge Inference

Always-on contextual AI runs language-aligned vision foundation models (VFMs) on edge devices, where the on-device model is the dominant continuous compute cost under strict latency and power limits. Due to an observed low-frequency shift in scene context and its relevant vocabulary, we present AdaDINO, an adaptive framework that makes on-device VFM inference efficient by matching execution to the current scene and task. We build on a known phenomenon, that the accuracy drop of shrinking model sizes depends on the task, and turn it into task-level adaptive execution. AdaDINO integrates neural architecture search (NAS) into a language-aligned VFM backbone distilled from DINOv2, training a single family of subnets for efficient execution during runtime. A multimodal large language model (LLM) on the cloud, invoked at low frequency, refines the candidate class set from scene context, while a learned selector activates the least-cost subnet predicted to retain a target fraction of accuracy. With the backbone and semantic pipeline held fixed, learned selection alone reduces average compute by $37\%$ over the best fixed subnet at equal segmentation accuracy. Across zero-shot classification and open-vocabulary segmentation, AdaDINO establishes a strong accuracy-efficiency frontier, improving over evaluated models of comparable sizes by up to $7.9\%$ in acc@1 on IN1K and $5.2\%$ mIoU on ADE20K, and reducing average FLOPs by up to $74.9\%$ at similar accuracy.

==> versions.tex <==
\providecommand{\paperversion}{arxiv}    %

\makeatletter
\def\pv@paper{paper}\def\pv@supp{supp}\def\pv@both{both}\def\pv@arxiv{arxiv}
\edef\pv@cur{\paperversion}
\newif\ifshowmain     %
\newif\ifshowsupp     %
\newif\ifsplitparts   %
\newif\ifarxiv        %
\ifx\pv@cur\pv@paper
  \showmaintrue  \showsuppfalse \splitpartsfalse \arxivfalse
\else\ifx\pv@cur\pv@supp
  \showmainfalse \showsupptrue  \splitpartsfalse \arxivfalse
\else\ifx\pv@cur\pv@both
  \showmaintrue  \showsupptrue  \splitpartstrue  \arxivfalse
\else\ifx\pv@cur\pv@arxiv
  \showmaintrue  \showsupptrue  \splitpartsfalse \arxivtrue
\else
  \PackageError{versions}{Unknown \string\paperversion='\paperversion'}%
    {Set \string\paperversion\space to one of: paper, supp, both, arxiv.}%
\fi\fi\fi\fi
\makeatother

\newcommand{\xv}[2]{\ifarxiv#2\else#1\fi}
\newcommand{\splitonly}[1]{\ifarxiv\else#1\fi}
\newcommand{\arxivonly}[1]{\ifarxiv#1\fi}

\newcommand{\suppref}[1]{\xv{\cref{#1} of the Supplementary Material}{\cref{#1}}}
\makeatletter
\long\def\snap@pad#1#2#3#4#5#6#7\snap@stop{%
  \global\expandafter\def\csname r@#1\endcsname{{#2}{#3}{#4}{#5}{#6}}}%
\newcommand{\snapinput}[1]{%
  \begingroup
    \def\newlabel##1##2{\snap@pad{##1}##2{}{}{}{}{}\snap@stop}%
    \input{#1}%
  \endgroup}
\makeatother
\ifshowmain\ifshowsupp\else
  \IfFileExists{supp-refs.tex}{%
    \snapinput{supp-refs}%
  }{%
    \PackageWarningNoLine{versions}{supp-refs.tex not found: \string\suppref\space
      references will print as ??. Run build/build.ps1 supp to regenerate it
      (and commit it so Overleaf sees it)}%
  }%
\fi\fi

\newcommand{\mainref}[1]{\xv{\cref{#1} of the main paper}{\cref{#1}}}
\ifshowmain\else\ifshowsupp
  \IfFileExists{main-refs.tex}{%
    \snapinput{main-refs}%
  }{%
    \PackageWarningNoLine{versions}{main-refs.tex not found: \string\mainref\space
      references will print as ??. Run build/build.ps1 paper to regenerate it
      (and commit it so Overleaf sees it)}%
  }%
\fi\fi

